Adaptive Ergodic Search with Energy-Aware Scheduling for Persistent Multi-Robot Missions

Autonomous robots are increasingly deployed for long-term information-gathering tasks, which pose two key challenges: planning informative trajectories in environments that evolve across space and time, and ensuring persistent operation under energy constraints. This paper presents a unified framework, mEclares, that addresses both challenges through adaptive ergodic search and energy-aware scheduling in multi-robot systems. Our contributions are two-fold: (1) we model real-world variability using stochastic spatiotemporal environments, where the underlying information evolves unpredictably due to process uncertainty. To guide exploration, we construct a target information spatial distribution (TISD) based on clarity, a metric that captures the decay of information in the absence of observations and highlights regions of high uncertainty; and (2) we introduce Robustmesch (Rmesch), an online scheduling method that enables persistent operation by coordinating rechargeable robots sharing a single mobile charging station. Unlike prior work, our approach avoids reliance on preplanned schedules, static or dedicated charging stations, and simplified robot dynamics. Instead, the scheduler supports general nonlinear models, accounts for uncertainty in the estimated position of the charging station, and handles central node failures. The proposed framework is validated through real-world hardware experiments, and feasibility guarantees are provided under specific assumptions.

==> subsections/intro.tex <==
% Autonomous robots are widely deployed in missions that require data acquisition over extended time horizons. Examples include environmental monitoring~(\cite{water_exploration1, water_exploration2}), ocean current characterization~(\cite{gulf1, gulf2}), wildfire surveillance~(\cite{julian2019distributed}), and search-and-rescue operations~(\cite{search_rescue1, search_rescue2}). Planning informative trajectories for such missions poses a diverse set of challenges. In this paper, we focus on two primary challenges: (i) how to plan robot trajectories that maximize the acquisition of relevant information in dynamic, evolving environments, and (ii) how to ensure task persistence by enabling robots to operate under energy constraints and return for recharging when necessary.

% The first challenge involves planning adaptive trajectories in spatiotemporal environments—where quantities of interest (e.g., temperature, wind speed, gas concentration) evolve over both space and time. Recent methods in ergodic search~(\cite{Mezic_Ergodic, Dressel_Ergodic, abraham2021ergodic, cmu_ergodic, dong2023time}) consider the spatial distribution of information when generating informative trajectories. This is achieved by constructing a target information spatial distribution (TISD) over the environment and adjusting the time spent in different regions accordingly. However, these methods typically assume either a \textit{spatiostatic environment}~(\cite{Mezic_Ergodic, dong2023time}, where the information varies only in space, or a spatiotemporal environment with a known model of variation~(\cite{Dressel_Ergodic, multiobjectiveergodic, Candela_thesis}). In many real-world scenarios, however, such variations are not fully predictable due to model mismatch, external disturbances, or inherent environmental variability.



% To account for this uncertainty, we consider a class of \textit{stochastic spatiotemporal environments}—spatiotemporal environments that exhibit process uncertainty in how they evolve over space and time. In general, stochastic variations in the environment can result in information decay without continuous monitoring. This motivates the need for online planning methods that adapt robot trajectories to changing information distributions and prioritize regions of high uncertainty and rapid information loss.

% The second challenge is task persistence under energy constraints. Robots must recharge to continue performing the mission, and coordination becomes especially important when multiple robots share a single charging station. Most prior work addresses this challenge by making simplifying assumptions. Some approaches assume each robot has access to a dedicated charging station~(\cite{dedicated_01, bentz2018complete}), while others consider static shared stations that allow multiple robots to recharge simultaneously~(\cite{static_charging_bipartite, singall_for_all_1, seewald2024energyaware}). Another class of methods precomputes rendezvous points before the mission begins, assuming robots follow fixed schedules to coordinate charging and information sharing~(\cite{pre-plan_1, pre-plan_2}). While these methods address important aspects of the problem, they also have limitations—some rely on simplified dynamics, such as single-integrator models~(\cite{persis_Fouad}), while others depend on preplanned trajectories or impose constraints on state-of-charge thresholds to manage coordination.

% In contrast, our framework does not rely on preplanned schedules, dedicated or static charging stations, or simplified robot dynamics. We develop an online scheduling method compatible with nonlinear robot models that enables exclusive use of a shared mobile charging station. The method accounts for uncertainty in the estimated position of the charging station. Although the proposed method is centralized, it provides a fail-safe maneuver at each decision epoch to ensure safe return in the event of central node failures or communication delays, while guaranteeing that robots do not deplete their energy below zero and arrive at the charging station at different times to avoid conflicts.

Autonomous robots are increasingly deployed in missions requiring long-term data acquisition, such as environmental monitoring~(\cite{water_exploration1, water_exploration2}), ocean current characterization~(\cite{gulf1, gulf2}), wildfire surveillance~(\cite{julian2019distributed}), and search-and-rescue operations~(\cite{search_rescue1, search_rescue2}). Planning informative trajectories for such missions poses two key challenges: (i) designing robot trajectories that maximize information acquisition in dynamic environments, and (ii) ensuring task persistence under energy constraints by enabling timely recharging.

The first challenge involves adaptive planning in spatiotemporal environments—where quantities of interest (e.g., temperature, wind speed, gas concentration) evolve across space and time. Ergodic search methods~(\cite{Mezic_Ergodic, Dressel_Ergodic, abraham2021ergodic}) address this by constructing a target information spatial distribution (TISD) and adjusting visitation time accordingly. However, existing approaches often assume a \textit{spatiostatic environment}~(\cite{Mezic_Ergodic, dong2023time}) or a spatiotemporal model with known variation(\cite{Dressel_Ergodic, Candela_thesis}), limiting their applicability in real-world settings where uncertainty arises from model mismatch, disturbances, or environmental variability.

To address this, we consider \textit{stochastic spatiotemporal environments}—environments whose evolution is uncertain in both space and time. In such cases, information can decay without continued measurement, motivating online trajectory planning that prioritizes regions with high uncertainty and rapid information loss.

The second challenge is persistent operation under energy constraints, particularly when multiple robots must coordinate recharging through a shared charging resource. Prior work often simplifies this problem: some assume each robot has a dedicated charging station~(\cite{dedicated_01, bentz2018complete}), others rely on static stations with multi-robot access at a time~(\cite{static_charging_bipartite, singall_for_all_1}), or preplanned rendezvous points~(\cite{pre-plan_1, pre-plan_2}) and fixed charging schedules. While these methods address important aspects of the problem, they also have limitations—some rely on simplified dynamics, such as single-integrator models~(\cite{persis_Fouad}), while others depend on preplanned trajectories or impose constraints on state-of-charge thresholds to manage coordination.

In contrast, our framework supports general nonlinear robot dynamics and enables online scheduling without relying on preplanned trajectories, static or dedicated charging stations. We take inspiration from work on safe planning through contingency~(\cite{gatekeeper, naveed2024mesch, naveed2025enabling, cherenson2025autonomy, tordesillas2019faster}) and propose a novel centralized scheduling method that ensures exclusive access to a shared mobile charging station while accounting for uncertainty in its estimated position. Additionally, our method plans a fail-safe maneuver at each decision point to guarantee safe returns under communication delays or central node failures, ensuring that robots never run out of energy and avoid return conflicts by arriving at different times.


% \textbf{\textit{Contributions:}}
% This paper introduces a unified framework for adaptive ergodic search with energy-aware scheduling in persistent multi-robot missions. The main contributions are as follows:  \textbf{1) Multi-agent principled TISD via clarity}: We construct the target information spatial distribution (TISD) using clarity~(\cite{clarity}), a bounded information metric that captures information decay and quantifies the maximum attainable information in stochastic spatiotemporal environments. As compared to our prior work~(\cite{naveed2024eclares}), we extend the clarity dynamics to the multi-agent setting to enable distributed sensing. 2) \textbf{Robust energy-aware multi-agent scheduling}: We propose a centralized online scheduling method, \Robustmesch{} (\Rmesch{}), that allocates recharging times to robots while accounting for general nonlinear dynamics and guaranteeing exclusive access to a shared mobile charging station. The method is robust to uncertainty in the estimated charger location and plans a fail-safe maneuver to ensure safe returns in the event of central node failures or communication delays, without violating energy constraints or causing conflicts. 3) \textbf{Hardware validation}: We validate the proposed framework through extensive simulations and real-world experiments using physical robots and a mobile charging platform.


% As compared to our previous conference papers~\cite{naveed2024eclares, naveed2024mesch}, this work provides several key extensions. Building on~\cite{naveed2024eclares}, we derive clarity dynamics for the multi-agent case, enabling distributed information acquisition. In contrast to~\cite{naveed2024mesch}, we introduce a fail-safe planner that ensures safe recovery under central node failures and communication delays, and we offer a more comprehensive analysis of the theoretical guarantees, including feasibility and robustness properties. Additionally, this work presents a significantly expanded experimental evaluation compared to the conference versions, including real-world hardware demonstrations where multiple aerial robots coordinate with a ground-based mobile charging station.

\textbf{\textit{Contributions:}}  
This paper introduces a unified framework for adaptive ergodic search with energy-aware scheduling in persistent multi-robot missions. The overall contributions are:

\begin{itemize}
    \item \textbf{Principled multi-agent TISD construction via clarity:}  
    We model the target information spatial distribution (TISD) using clarity~\cite{clarity}, a bounded metric that captures information decay and quantifies the maximum attainable information in stochastic spatiotemporal environments. This enables robots to adaptively focus sensing effort in regions with the highest informational value.

    \item \textbf{Robust energy-aware scheduling with fail-safe coordination:}  
    We propose \Robustmesch{} (\Rmesch{}), a centralized online scheduling framework that accounts for general nonlinear robot dynamics, enforces exclusive access to a shared mobile charging station, and guarantees safe returns even in the presence of central node failures or communication delays via a decentralized fail-safe planner.

    \item \textbf{Real-world experimental validation:}  
    We demonstrate the full framework on a heterogeneous team comprising multiple aerial robots and a mobile ground-based charging station through extensive hardware experiments and field trials.
\end{itemize}

\textbf{\textit{Comparison to prior conference works:}} Compared to our earlier conference papers, this work introduces several key extensions:
\begin{itemize}
    \item Compared to~\cite{naveed2024eclares}, we extend the clarity-based information model to the multi-agent case, enabling distributed sensing and coordination.
    \item Compared to~\cite{naveed2024mesch}, we introduce a fail-safe planner that enables safe recovery under central node failures and provide a more comprehensive theoretical analysis, including formal guarantees on feasibility and robustness.
    \item In addition, this paper presents an expanded experimental evaluation compared to both prior works, including real-world demonstrations involving multiple aerial robots coordinating through a shared mobile charging station.
\end{itemize}


% \subsubsection*{Contributions}
% This paper presents a unified framework for adaptive ergodic search with energy-aware scheduling in persistent multi-robot missions. The core contributions are:

% \begin{itemize}
%     \item \textbf{Multi-Agent Principled TISD via clarity}: We construct the target information spatial distribution (TISD) using clarity~\cite{clarity}, a bounded information measure that captures information decay due to lack of measurements and quantifies the maximum attainable information in stochastic spatiotemporal environments. We extend the clarity dynamics to the multi-agent case to support distributed sensing.
    
%     \item \textbf{Robust energy-aware multi-agent scheduling}: We develop a centralized online scheduling method, \Robustmesch{} (\Rmesch{}), that assigns recharging times while supporting general nonlinear robot dynamics and ensuring exclusive access to a shared mobile charging station. The method accounts for uncertainty in the estimated position of the charger and includes a fail-safe maneuver to ensure safe return under central node failures or communication delays, without violating minimum energy constraints or causing conflicts at the charging station.
    
%     \item \textbf{Hardware validation}: We demonstrate the effectiveness of the proposed framework through extensive simulations and real-world experiments using physical robots and a mobile charging platform.
% \end{itemize}







==> subsections/related.tex <==
\subsection{Adaptive Informative path planning}

Our work falls more broadly under the category of informative path planning (IPP). In IPP, robot paths are generated to maximize information gain or minimize uncertainty along the trajectory, subject to budget constraints. Classical approaches include orienteering-based formulations that select a subset of informative locations under path-length constraints~(\cite{bottarelli2019orienteering}), submodular optimization methods that leverage diminishing returns in information gain~(\cite{meliou2007nonmyopic}), and Gaussian Process (GP)-based planners that explicitly model spatial uncertainty~(\cite{Chen-RSS-22}). To improve scalability and adaptability, particularly in high-dimensional or continuous spaces—sampling-based planners~(\cite{moon2025ia}) and receding horizon strategies have been proposed~(\cite{sun2017no}). While each of these approaches has shown promise, many struggle with handling long planning horizons, real-time adaptability to variations in stochastic spatiotemporal environments. 

Ergodic search offers an alternative perspective by generating trajectories that match the time-averaged visitation frequency of the robot with a target information spatial distribution (TISD), rather than selecting a subset of discrete locations. Recent advances in ergodic exploration~(\cite{Mezic_Ergodic, Dressel_Ergodic, abraham2021ergodic, cmu_ergodic, dong2023time}) have shown the effectiveness of this approach in generating spatially balanced coverage trajectories. These methods typically construct a TISD over the environment and generate trajectories that spend more time in regions of higher information content. However, most prior work assumes either \emph{spatiostatic environments}~(\cite{Mezic_Ergodic, dong2023time}), where the information only varies spatially, or environments with known spatiotemporal dynamics~(\cite{Dressel_Ergodic, multiobjectiveergodic, Candela_thesis}). As a result, they cannot account for stochastic variation or capture information decay that naturally arises in unobserved regions over time. To address this limitation, we build on the clarity metric~(\cite{clarity}), a bounded information measure between $[0,1]$ that captures information loss due to lack of observations and quantifies the maximum attainable information in stochastic spatiotemporal environments. Using clarity, we construct a principled TISD that continuously evolves based on the robot's measurement history and environmental uncertainty.

In this work, we address this gap by constructing the TISD using clarity, a bounded information measure that captures both current knowledge and its decay over time. This allows the robot to adaptively revisit regions where uncertainty is increasing.
 

\subsection{Task Persistence in Multi-Agent Systems}
\label{sec:related_work_task_persistence}


Recent work on task persistence spans both single-agent and multi-agent settings, with studies exploring scenarios involving \emph{static} and \emph{mobile} charging infrastructure.

For static stations, prior work typically assumes either a dedicated charger per robot~\cite{dedicated_01, dedicated_02, dedicated_03, multirobot_game_theoretic}, or a shared charger capable of recharging multiple agents simultaneously~\cite{singall_for_all_1, periodic_charging}. Other approaches consider fewer stations than robots~\cite{static_charging_bipartite, static_placing_charging, seewald2024energyaware}, and ensure energy availability by modifying mission paths~\cite{static_charging_bipartite}, strategically placing stations~\cite{static_placing_charging}, or constraining the number of robots that return for charging~\cite{seewald2024energyaware}.

We focus on a setting where all robots share a \emph{single} charging station exclusively. Closest prior works are~\cite{bentz2018complete, persis_Fouad}. In~\cite{bentz2018complete}, exclusivity is achieved by staggering deployments, while~\cite{persis_Fouad} uses control barrier functions (CBFs)~\cite{CBF_TAC} to regulate minimum SoC under single-integrator dynamics. In contrast, our online scheduling algorithm ensures exclusive access without requiring deployment delays or specific battery configurations. Our method applies to nonlinear robot models and extends naturally to mobile charging scenarios.

Most mobile charging approaches assume that one robot within the network acts as a charger. Some methods precompute rendezvous points offline~\cite{pre-plan_1, pre-plan_2}, while others rely on continuous communication for online coordination~\cite{continous_comms_1}. Alternatively, some works deploy dedicated charging robots that intercept mission paths~\cite{cooperative_1, cooperative_2, MOBILE_RAL_2022}. In this work, we consider a mobile charging robot that facilitates the operation of rechargeable robots. We plan the trajectory of the mobile charging station so that it travels alongside the network of rechargeable robots, extending their operational time. Our framework enables energy-aware task persistence without relying on preplanned rendezvous. 

